Follow-up on three poorly studied AM CVn stars

We report follow-up observations of three poorly studied AM CVn-type binaries: CRTS CSS150211 J091017-200813, NSV1440, and SDSSJ183131.63+420220.2. Analysing time-series photometry obtained with a range of ground-based facilities as well as with TESS, we determine the superhump period of CRTSJ0910-2008 as P_sh=29.700+-0.004min and the orbital period of NSV1440 as Porb=36.56+-0.03min. We also confirm a photometric period of P=23.026+-0.097min in SDSSJ1831+4202, which is most likely the superhump period. We also report the first optical spectroscopy of CRTSJ0910-2008 and NSV1440 which unambiguously confirms both as AM CVn systems. We briefly discuss the distribution in the Hertzsprung-Russell diagram of the currently known sample of 63 AM CVn stars with known periods and Gaia data.

==> bibliography.tex <==
\begin{thebibliography}{}
\makeatletter
\relax
\def\mn@urlcharsother{\let\do\@makeother \do\$\do\&\do\#\do\^\do\_\do\%\do\~}
\def\mn@doi{\begingroup\mn@urlcharsother \@ifnextchar [ {\mn@doi@} {\mn@doi@[]}}
\def\mn@doi@[#1]#2{\def\@tempa{#1}\ifx\@tempa\@empty \href {http://dx.doi.org/#2} {doi:#2}\else \href {http://dx.doi.org/#2} {#1}\fi \endgroup}
\def\mn@eprint#1#2{\mn@eprint@#1:#2::\@nil}
\def\mn@eprint@arXiv#1{\href {http://arxiv.org/abs/#1} {{\tt arXiv:#1}}}
\def\mn@eprint@dblp#1{\href {http://dblp.uni-trier.de/rec/bibtex/#1.xml} {dblp:#1}}
\def\mn@eprint@#1:#2:#3:#4\@nil{\def\@tempa {#1}\def\@tempb {#2}\def\@tempc {#3}\ifx \@tempc \@empty \let \@tempc \@tempb \let \@tempb \@tempa \fi \ifx \@tempb \@empty \def\@tempb {arXiv}\fi \@ifundefined {mn@eprint@\@tempb}{\@tempb:\@tempc}{\expandafter \expandafter \csname mn@eprint@\@tempb\endcsname \expandafter{\@tempc}}}

\bibitem[\protect\citeauthoryear{{Amaro-Seoane} et~al.,}{{Amaro-Seoane} et~al.}{2012}]{amaro-seoaneetal12-1}
{Amaro-Seoane} P.,  et~al., 2012, \mn@doi [Classical and Quantum Gravity] {10.1088/0264-9381/29/12/124016}, \href {https://ui.adsabs.harvard.edu/abs/2012CQGra..29l4016A} {29, 124016}

\bibitem[\protect\citeauthoryear{{Bellm} et~al.,}{{Bellm} et~al.}{2019}]{bellmetal19-1}
{Bellm} E.~C.,  et~al., 2019, \mn@doi [PASP] {10.1088/1538-3873/aaecbe}, \href {https://ui.adsabs.harvard.edu/abs/2019PASP..131a8002B} {131, 018002}

\bibitem[\protect\citeauthoryear{{Bertin} \& {Arnouts}}{{Bertin} \& {Arnouts}}{1996}]{bertin+arnouts96-1}
{Bertin} E.,  {Arnouts} S.,  1996, A\&AS, \href {https://ui.adsabs.harvard.edu/abs/1996A&AS..117..393B} {117, 393}

\bibitem[\protect\citeauthoryear{{Bildsten}, {Shen}, {Weinberg}  \& {Nelemans}}{{Bildsten} et~al.}{2007}]{bildstenetal07-1}
{Bildsten} L.,  {Shen} K.~J.,  {Weinberg} N.~N.,   {Nelemans} G.,  2007, \mn@doi [ApJ Lett.] {10.1086/519489}, \href {https://ui.adsabs.harvard.edu/abs/2007ApJ...662L..95B} {662, L95}

\bibitem[\protect\citeauthoryear{{Carter} et~al.,}{{Carter} et~al.}{2013}]{carteretal13-1}
{Carter} P.~J.,  et~al., 2013, \mn@doi [MNRAS] {10.1093/mnras/sts485}, \href {https://ui.adsabs.harvard.edu/abs/2013MNRAS.429.2143C} {429, 2143}

\bibitem[\protect\citeauthoryear{{Clemens}, {Crain}  \& {Anderson}}{{Clemens} et~al.}{2004}]{clemensetal04-1}
{Clemens} J.~C.,  {Crain} J.~A.,   {Anderson} R.,  2004, in {Moorwood} A. F.~M.,  {Iye} M.,  eds,  Proceedings of SPIE Vol. 5492, Ground-based Instrumentation for Astronomy. pp 331--340, \mn@doi{10.1117/12.550069}

\bibitem[\protect\citeauthoryear{{Currie}, {Berry}, {Jenness}, {Gibb}, {Bell}  \& {Draper}}{{Currie} et~al.}{2014}]{currieetal14-1}
{Currie} M.~J.,  {Berry} D.~S.,  {Jenness} T.,  {Gibb} A.~G.,  {Bell} G.~S.,   {Draper} P.~W.,  2014, in {Manset} N.,  {Forshay} P.,  eds, Astronomical Data Analysis Software and Systems XXIII. ASP Conf. Ser. 485, p.~391

\bibitem[\protect\citeauthoryear{{Dhillon} et~al.,}{{Dhillon} et~al.}{2007}]{dhillonetal07-1}
{Dhillon} V.~S.,  et~al., 2007, \mn@doi [MNRAS] {10.1111/j.1365-2966.2007.11881.x}, \href {https://ui.adsabs.harvard.edu/abs/2007MNRAS.378..825D} {378, 825}

\bibitem[\protect\citeauthoryear{{Dhillon} et~al.,}{{Dhillon} et~al.}{2014}]{dhillonetal14-1}
{Dhillon} V.~S.,  et~al., 2014, \mn@doi [MNRAS] {10.1093/mnras/stu1660}, \href {https://ui.adsabs.harvard.edu/abs/2014MNRAS.444.4009D} {444, 4009}

\bibitem[\protect\citeauthoryear{{Drake} et~al.,}{{Drake} et~al.}{2009}]{drakeetal09-1}
{Drake} A.~J.,  et~al., 2009, \mn@doi [ApJ] {10.1088/0004-637X/696/1/870}, \href {https://ui.adsabs.harvard.edu/abs/2009ApJ...696..870D} {696, 870}

\bibitem[\protect\citeauthoryear{{Duffy} et~al.,}{{Duffy} et~al.}{2021}]{duffyetal21-1}
{Duffy} C.,  et~al., 2021, \mn@doi [MNRAS] {10.1093/mnras/stab389}, \href {https://ui.adsabs.harvard.edu/abs/2021MNRAS.502.4953D} {502, 4953}

\bibitem[\protect\citeauthoryear{{Gaia Collaboration} et~al.,}{{Gaia Collaboration} et~al.}{2018}]{gaiaetal18-1}
{Gaia Collaboration} et~al., 2018, \mn@doi [A\&A] {10.1051/0004-6361/201833051}, \href {https://ui.adsabs.harvard.edu/abs/2018A&A...616A...1G} {616, A1}

\bibitem[\protect\citeauthoryear{{G{\"a}nsicke} et~al.,}{{G{\"a}nsicke} et~al.}{2003}]{gaensickeetal03-1}
{G{\"a}nsicke} B.~T.,  et~al., 2003, ApJ, \href {https://ui.adsabs.harvard.edu/abs/2003ApJ...594..443G} {594, 443}

\bibitem[\protect\citeauthoryear{Green}{Green}{2023}]{green23-1}
Green M.,  2023, \mn@doi [Zenodo] {10.5281/zenodo.12672892}

\bibitem[\protect\citeauthoryear{{Green} et~al.,}{{Green} et~al.}{2018}]{greenetal18-1}
{Green} M.~J.,  et~al., 2018, \mn@doi [MNRAS] {10.1093/mnras/sty1032}, \href {https://ui.adsabs.harvard.edu/abs/2018MNRAS.477.5646G} {477, 5646}

\bibitem[\protect\citeauthoryear{{Green} et~al.,}{{Green} et~al.}{2020}]{greenetal20-1}
{Green} M.~J.,  et~al., 2020, \mn@doi [MNRAS] {10.1093/mnras/staa1509}, \href {https://ui.adsabs.harvard.edu/abs/2020MNRAS.496.1243G} {496, 1243}

\bibitem[\protect\citeauthoryear{{Green} et~al.,}{{Green} et~al.}{2024}]{greenetal24-1}
{Green} M.~J.,  et~al., 2024, \mn@doi [MNRAS] {10.1093/mnras/stad3412}, \href {https://ui.adsabs.harvard.edu/abs/2024MNRAS.527.3445G} {527, 3445}

\bibitem[\protect\citeauthoryear{{Greenstein} \& {Matthews}}{{Greenstein} \& {Matthews}}{1957}]{greenstein+matthews57-1}
{Greenstein} J.~L.,  {Matthews} M.~S.,  1957, \mn@doi [ApJ] {10.1086/146364}, \href {https://ui.adsabs.harvard.edu/abs/1957ApJ...126...14G} {126, 14}

\bibitem[\protect\citeauthoryear{{Hardy} et~al.,}{{Hardy} et~al.}{2017}]{hardyetal17-1}
{Hardy} L.~K.,  et~al., 2017, \mn@doi [MNRAS] {10.1093/mnras/stw3051}, \href {https://ui.adsabs.harvard.edu/abs/2017MNRAS.465.4968H} {465, 4968}

\bibitem[\protect\citeauthoryear{{Iben} \& {Tutukov}}{{Iben} \& {Tutukov}}{1987}]{iben+tutukov87-1}
{Iben} Jr. I.,  {Tutukov} A.~V.,  1987, \mn@doi [ApJ] {10.1086/165011}, \href {https://ui.adsabs.harvard.edu/abs/1987ApJ...313..727I} {313, 727}

\bibitem[\protect\citeauthoryear{{Inight} et~al.,}{{Inight} et~al.}{2022}]{inightetal22-1}
{Inight} K.,  et~al., 2022, \mn@doi [MNRAS] {10.1093/mnras/stab3662}, \href {https://ui.adsabs.harvard.edu/abs/2022MNRAS.510.3605I} {510, 3605}

\bibitem[\protect\citeauthoryear{{Inight} et~al.,}{{Inight} et~al.}{2023}]{inightetal23-1}
{Inight} K.,  et~al., 2023, \mn@doi [MNRAS] {10.1093/mnras/stad2018}, \href {https://ui.adsabs.harvard.edu/abs/2023MNRAS.524.4867I} {524, 4867}

\bibitem[\protect\citeauthoryear{{Isogai}, {Kato}, {Monard}, {Hambsch}, {Myers}, {Starr}, {Cook}  \& {Nogami}}{{Isogai} et~al.}{2019}]{isogaietal19-1}
{Isogai} K.,  {Kato} T.,  {Monard} B.,  {Hambsch} F.-J.,  {Myers} G.,  {Starr} P.,  {Cook} L.~M.,   {Nogami} D.,  2019, \mn@doi [\pasj] {10.1093/pasj/psz018}, \href {https://ui.adsabs.harvard.edu/abs/2019PASJ...71...48I} {71, 48}

\bibitem[\protect\citeauthoryear{{Kato}}{{Kato}}{2015}]{kato15-1}
{Kato} T.,  2015, \mn@doi [\pasj] {10.1093/pasj/psv077}, \href {https://ui.adsabs.harvard.edu/abs/2015PASJ...67..108K} {67, 108}

\bibitem[\protect\citeauthoryear{{Kato}}{{Kato}}{2023}]{kato23-1}
{Kato} T.,  2023, \mn@doi [arXiv e-prints] {10.48550/arXiv.2307.08954}, \href {https://ui.adsabs.harvard.edu/abs/2023arXiv230708954K} {p. arXiv:2307.08954}

\bibitem[\protect\citeauthoryear{{Kato} \& {Osaki}}{{Kato} \& {Osaki}}{2013}]{kato+osaki13-1}
{Kato} T.,  {Osaki} Y.,  2013, \mn@doi [PASJ] {10.1093/pasj/65.5.97}, \href {https://ui.adsabs.harvard.edu/abs/2013PASJ...65...97K} {65, 97}

\bibitem[\protect\citeauthoryear{{Kato} \& {Stubbings}}{{Kato} \& {Stubbings}}{2023}]{kato+stubbings23-1}
{Kato} T.,  {Stubbings} R.,  2023, \mn@doi [VSOLJ Variable Star Bulletin] {10.48550/arXiv.2305.04194}, \href {https://ui.adsabs.harvard.edu/abs/2023arXiv230504194K} {116, arXiv:2305.04194}

\bibitem[\protect\citeauthoryear{{Kato}, {Hachisu}, {Kiyota}  \& {Saio}}{{Kato} et~al.}{2008}]{katoetal08-1}
{Kato} M.,  {Hachisu} I.,  {Kiyota} S.,   {Saio} H.,  2008, \mn@doi [ApJ] {10.1086/590329}, \href {https://ui.adsabs.harvard.edu/abs/2008ApJ...684.1366K} {684, 1366}

\bibitem[\protect\citeauthoryear{{Kato} et~al.,}{{Kato} et~al.}{2009}]{katoetal09-1}
{Kato} T.,  et~al., 2009, PASJ, \href {https://ui.adsabs.harvard.edu/abs/2009PASJ...61S.395K} {61, 395}

\bibitem[\protect\citeauthoryear{{Khalil} et~al.,}{{Khalil} et~al.}{2024}]{khaliletal24-1}
{Khalil} J.~M.,  et~al., 2024, \mn@doi [A\&A] {10.1051/0004-6361/202349010}, \href {https://ui.adsabs.harvard.edu/abs/2024A&A...683L..10K} {683, L10}

\bibitem[\protect\citeauthoryear{{Kochanek} et~al.,}{{Kochanek} et~al.}{2017}]{kochaneketal17-1}
{Kochanek} C.~S.,  et~al., 2017, \mn@doi [PASP] {10.1088/1538-3873/aa80d9}, \href {https://ui.adsabs.harvard.edu/abs/2017PASP..129j4502K} {129, 104502}

\bibitem[\protect\citeauthoryear{{Korol}, {Rossi}, {Groot}, {Nelemans}, {Toonen}  \& {Brown}}{{Korol} et~al.}{2017}]{koroletal17-1}
{Korol} V.,  {Rossi} E.~M.,  {Groot} P.~J.,  {Nelemans} G.,  {Toonen} S.,   {Brown} A.~G.~A.,  2017, \mn@doi [MNRAS] {10.1093/mnras/stx1285}, \href {https://ui.adsabs.harvard.edu/abs/2017MNRAS.470.1894K} {470, 1894}

\bibitem[\protect\citeauthoryear{{Kotko}, {Lasota}, {Dubus}  \& {Hameury}}{{Kotko} et~al.}{2012}]{kotkoetal12-1}
{Kotko} I.,  {Lasota} J.-P.,  {Dubus} G.,   {Hameury} J.-M.,  2012, \mn@doi [A\&A] {10.1051/0004-6361/201219156}, \href {https://ui.adsabs.harvard.edu/abs/2012A&A...544A..13K} {544, A13}

\bibitem[\protect\citeauthoryear{{Kupfer} et~al.,}{{Kupfer} et~al.}{2018}]{kupferetal18-1}
{Kupfer} T.,  et~al., 2018, \mn@doi [MNRAS] {10.1093/mnras/sty1545}, \href {https://ui.adsabs.harvard.edu/abs/2018MNRAS.480..302K} {480, 302}

\bibitem[\protect\citeauthoryear{{Levitan} et~al.,}{{Levitan} et~al.}{2011}]{levitanetal11-1}
{Levitan} D.,  et~al., 2011, \mn@doi [ApJ] {10.1088/0004-637X/739/2/68}, \href {https://ui.adsabs.harvard.edu/abs/2011ApJ...739...68L} {739, 68}

\bibitem[\protect\citeauthoryear{{Levitan}, {Groot}, {Prince}, {Kulkarni}, {Laher}, {Ofek}, {Sesar}  \& {Surace}}{{Levitan} et~al.}{2015}]{levitanetal15-1}
{Levitan} D.,  {Groot} P.~J.,  {Prince} T.~A.,  {Kulkarni} S.~R.,  {Laher} R.,  {Ofek} E.~O.,  {Sesar} B.,   {Surace} J.,  2015, \mn@doi [MNRAS] {10.1093/mnras/stu2105}, \href {https://ui.adsabs.harvard.edu/abs/2015MNRAS.446..391L} {446, 391}

\bibitem[\protect\citeauthoryear{{Marsh}}{{Marsh}}{1989}]{marsh89-1}
{Marsh} T.~R.,  1989, PASP, \href {https://ui.adsabs.harvard.edu/abs/1989PASP..101.1032M} {101, 1032}

\bibitem[\protect\citeauthoryear{{Marsh}, {Nelemans}  \& {Steeghs}}{{Marsh} et~al.}{2004}]{marshetal04-1}
{Marsh} T.~R.,  {Nelemans} G.,   {Steeghs} D.,  2004, \mn@doi [MNRAS] {10.1111/j.1365-2966.2004.07564.x}, \href {https://ui.adsabs.harvard.edu/abs/2004MNRAS.350..113M} {350, 113}

\bibitem[\protect\citeauthoryear{{Masci} et~al.,}{{Masci} et~al.}{2019}]{mascietal19-1}
{Masci} F.~J.,  et~al., 2019, \mn@doi [PASP] {10.1088/1538-3873/aae8ac}, \href {https://ui.adsabs.harvard.edu/abs/2019PASP..131a8003M} {131, 018003}

\bibitem[\protect\citeauthoryear{{Nelemans}, {Yungelson}  \& {Portegies Zwart}}{{Nelemans} et~al.}{2004}]{nelemansetal04-1}
{Nelemans} G.,  {Yungelson} L.~R.,   {Portegies Zwart} S.~F.,  2004, \mn@doi [MNRAS] {10.1111/j.1365-2966.2004.07479.x}, \href {https://ui.adsabs.harvard.edu/abs/2004MNRAS.349..181N} {349, 181}

\bibitem[\protect\citeauthoryear{{Nelemans}, {Yungelson}, {van der Sluys}  \& {Tout}}{{Nelemans} et~al.}{2010}]{nelemansetal10-1}
{Nelemans} G.,  {Yungelson} L.~R.,  {van der Sluys} M.~V.,   {Tout} C.~A.,  2010, \mn@doi [MNRAS] {10.1111/j.1365-2966.2009.15731.x}, \href {https://ui.adsabs.harvard.edu/abs/2010MNRAS.401.1347N} {401, 1347}

\bibitem[\protect\citeauthoryear{{Osaki}}{{Osaki}}{1974}]{osaki74-1}
{Osaki} Y.,  1974, \pasj, \href {https://ui.adsabs.harvard.edu/abs/1974PASJ...26..429O} {26, 429}

\bibitem[\protect\citeauthoryear{{Paczy{\'n}ski}}{{Paczy{\'n}ski}}{1967}]{paczynski67-1}
{Paczy{\'n}ski} B.,  1967, \actaa, \href {https://ui.adsabs.harvard.edu/abs/1967AcA....17..287P} {17, 287}

\bibitem[\protect\citeauthoryear{{Patterson} et~al.,}{{Patterson} et~al.}{2005}]{pattersonetal05-3}
{Patterson} J.,  et~al., 2005, \mn@doi [PASP] {10.1086/447771}, \href {https://ui.adsabs.harvard.edu/abs/2005PASP..117.1204P} {117, 1204}

\bibitem[\protect\citeauthoryear{{Podsiadlowski}, {Han}  \& {Rappaport}}{{Podsiadlowski} et~al.}{2003}]{podsiadlowskietal03-1}
{Podsiadlowski} P.,  {Han} Z.,   {Rappaport} S.,  2003, MNRAS, \href {https://ui.adsabs.harvard.edu/abs/2003MNRAS.340.1214P} {340, 1214}

\bibitem[\protect\citeauthoryear{{Ramsay}, {Barclay}, {Steeghs}, {Wheatley}, {Hakala}, {Kotko}  \& {Rosen}}{{Ramsay} et~al.}{2012}]{ramsayetal12-2}
{Ramsay} G.,  {Barclay} T.,  {Steeghs} D.,  {Wheatley} P.~J.,  {Hakala} P.,  {Kotko} I.,   {Rosen} S.,  2012, \mn@doi [MNRAS] {10.1111/j.1365-2966.2011.19924.x}, \href {https://ui.adsabs.harvard.edu/abs/2012MNRAS.419.2836R} {419, 2836}

\bibitem[\protect\citeauthoryear{{Ramsay} et~al.,}{{Ramsay} et~al.}{2018}]{ramsayetal18-1}
{Ramsay} G.,  et~al., 2018, \mn@doi [A\&A] {10.1051/0004-6361/201834261}, \href {https://ui.adsabs.harvard.edu/abs/2018A&A...620A.141R} {620, A141}

\bibitem[\protect\citeauthoryear{{Rivera Sandoval}, {Maccarone}  \& {Pichardo Marcano}}{{Rivera Sandoval} et~al.}{2020}]{riverasandovaletal20-1}
{Rivera Sandoval} L.~E.,  {Maccarone} T.~J.,   {Pichardo Marcano} M.,  2020, \mn@doi [ApJ Lett.] {10.3847/2041-8213/abb130}, \href {https://ui.adsabs.harvard.edu/abs/2020ApJ...900L..37R} {900, L37}

\bibitem[\protect\citeauthoryear{{Rivera Sandoval}, {Maccarone}, {Cavecchi}, {Britt}  \& {Zurek}}{{Rivera Sandoval} et~al.}{2021}]{riverasandovaletal21-1}
{Rivera Sandoval} L.~E.,  {Maccarone} T.~J.,  {Cavecchi} Y.,  {Britt} C.,   {Zurek} D.,  2021, \mn@doi [MNRAS] {10.1093/mnras/stab1246}, \href {https://ui.adsabs.harvard.edu/abs/2021MNRAS.505..215R} {505, 215}

\bibitem[\protect\citeauthoryear{{Rivera Sandoval}, {Heinke}, {Hameury}, {Cavecchi}, {Vanmunster}, {Tordai}  \& {Romanov}}{{Rivera Sandoval} et~al.}{2022}]{riverasandovaletal22-1}
{Rivera Sandoval} L.~E.,  {Heinke} C.~O.,  {Hameury} J.~M.,  {Cavecchi} Y.,  {Vanmunster} T.,  {Tordai} T.,   {Romanov} F.~D.,  2022, \mn@doi [ApJ] {10.3847/1538-4357/ac3fb7}, \href {https://ui.adsabs.harvard.edu/abs/2022ApJ...926...10R} {926, 10}

\bibitem[\protect\citeauthoryear{{Rodriguez} et~al.,}{{Rodriguez} et~al.}{2023}]{rodriguezetal23-1}
{Rodriguez} A.~C.,  et~al., 2023, \mn@doi [ApJ] {10.3847/1538-4357/ace698}, \href {https://ui.adsabs.harvard.edu/abs/2023ApJ...954...63R} {954, 63}

\bibitem[\protect\citeauthoryear{{Savonije}, {de Kool}  \& {van den Heuvel}}{{Savonije} et~al.}{1986}]{savonijeetal86-1}
{Savonije} G.~J.,  {de Kool} M.,   {van den Heuvel} E.~P.~J.,  1986, A\&A, \href {https://ui.adsabs.harvard.edu/abs/1986A&A...155...51S} {155, 51}

\bibitem[\protect\citeauthoryear{{Scargle}}{{Scargle}}{1982}]{scargle82-1}
{Scargle} J.~D.,  1982, ApJ, \href {https://ui.adsabs.harvard.edu/abs/1982ApJ...263..835S} {263, 835}

\bibitem[\protect\citeauthoryear{{Shappee} et~al.,}{{Shappee} et~al.}{2014}]{shappeeetal14-1}
{Shappee} B.~J.,  et~al., 2014, \mn@doi [ApJ] {10.1088/0004-637X/788/1/48}, \href {https://ui.adsabs.harvard.edu/abs/2014ApJ...788...48S} {788, 48}

\bibitem[\protect\citeauthoryear{{Shen} \& {Bildsten}}{{Shen} \& {Bildsten}}{2014}]{shen+bildsten14-1}
{Shen} K.~J.,  {Bildsten} L.,  2014, \mn@doi [ApJ] {10.1088/0004-637X/785/1/61}, \href {https://ui.adsabs.harvard.edu/abs/2014ApJ...785...61S} {785, 61}

\bibitem[\protect\citeauthoryear{{Smak}}{{Smak}}{1967}]{smak67-1}
{Smak} J.,  1967, \actaa, \href {https://ui.adsabs.harvard.edu/abs/1967AcA....17..255S} {17, 255}

\bibitem[\protect\citeauthoryear{{Solheim}}{{Solheim}}{2010}]{solheim10-1}
{Solheim} J.,  2010, \mn@doi [PASP] {10.1086/656680}, \href {https://ui.adsabs.harvard.edu/abs/2010PASP..122.1133S} {122, 1133}

\bibitem[\protect\citeauthoryear{{Steeghs} et~al.,}{{Steeghs} et~al.}{2022}]{steeghsetal22-1}
{Steeghs} D.,  et~al., 2022, \mn@doi [MNRAS] {10.1093/mnras/stac013}, \href {https://ui.adsabs.harvard.edu/abs/2022MNRAS.511.2405S} {511, 2405}

\bibitem[\protect\citeauthoryear{{Toloza} et~al.,}{{Toloza} et~al.}{2019}]{tolozaetal19-1}
{Toloza} O.,  et~al., 2019, in Bulletin of the American Astronomical Society. p.~168

\bibitem[\protect\citeauthoryear{{Watson}, {Henden}  \& {Price}}{{Watson} et~al.}{2006}]{watsonetal16-1}
{Watson} C.~L.,  {Henden} A.~A.,   {Price} A.,  2006, Society for Astronomical Sciences Annual Symposium, \href {https://ui.adsabs.harvard.edu/abs/2006SASS...25...47W} {25, 47}

\bibitem[\protect\citeauthoryear{{Whitehurst} \& {King}}{{Whitehurst} \& {King}}{1991}]{whitehurst+king91-1}
{Whitehurst} R.,  {King} A.,  1991, MNRAS, \href {https://ui.adsabs.harvard.edu/abs/1991MNRAS.249...25W} {249, 25}

\bibitem[\protect\citeauthoryear{{Woudt} et~al.,}{{Woudt} et~al.}{2009}]{woudtetal09-1}
{Woudt} P.~A.,  et~al., 2009, \mn@doi [ApJ] {10.1088/0004-637X/706/1/738}, \href {https://ui.adsabs.harvard.edu/abs/2009ApJ...706..738W} {706, 738}

\bibitem[\protect\citeauthoryear{{Yamaguchi}, {El-Badry}, {Rodriguez}, {Gull}, {Roulston}  \& {Vanderbosch}}{{Yamaguchi} et~al.}{2023}]{yamaguchietal23-1}
{Yamaguchi} N.,  {El-Badry} K.,  {Rodriguez} A.~C.,  {Gull} M.,  {Roulston} B.~R.,   {Vanderbosch} Z.~P.,  2023, \mn@doi [MNRAS] {10.1093/mnras/stad1878}, \href {https://ui.adsabs.harvard.edu/abs/2023MNRAS.524..740Y} {524, 740}

\bibitem[\protect\citeauthoryear{{van Roestel} et~al.,}{{van Roestel} et~al.}{2021}]{vanroesteletal21-1}
{van Roestel} J.,  et~al., 2021, \mn@doi [AJ] {10.3847/1538-3881/ac0622}, \href {https://ui.adsabs.harvard.edu/abs/2021AJ....162..113V} {162, 113}

\bibitem[\protect\citeauthoryear{{van Roestel} et~al.,}{{van Roestel} et~al.}{2022}]{vanroesteletal22-1}
{van Roestel} J.,  et~al., 2022, \mn@doi [MNRAS] {10.1093/mnras/stab2421}, \href {https://ui.adsabs.harvard.edu/abs/2022MNRAS.512.5440V} {512, 5440}

\makeatother
\end{thebibliography}

